Spark: A System for Scientifically Creative Idea Generation

Recently, large language models (LLMs) have shown promising abilities to generate novel research ideas in science, a direction which coincides with many foundational principles in computational creativity (CC). In light of these developments, we present an idea generation system named Spark that couples retrieval-augmented idea generation using LLMs with a reviewer model named Judge trained on 600K scientific reviews from OpenReview. Our work is both a system demonstration and intended to inspire other CC researchers to explore grounding the generation and evaluation of scientific ideas within foundational CC principles. To this end, we release the annotated dataset used to train Judge, inviting other researchers to explore the use of LLMs for idea generation and creative evaluations.

==> figures/xplor_prompts.tex <==
\begin{figure}[ht]
  \centering
  \footnotesize
  \begin{minipage}{\columnwidth}
    \color{blacktext} % Default text color

    % --- Section A ---
    \sectiontitlegreen{A) Inputs:}
    \begin{itemize} \itemsep -0.2em % Tighter item separation
      \item \textbf{Question:} \\ \texttt{"LLM reasoning consistency?"}
      \item \textbf{Source:} \texttt{Papers} or \texttt{Search Flag}
    \end{itemize}
    % Removed vspace

    % --- Section B ---
    \sectiontitlegreen{B) Relevance Scoring Prompt (per chunk):}
    % Use tcolorbox for light green background and black text
    \begin{tcolorbox}[colback=lightgreenbg, coltext=blacktext, boxrule=0pt, arc=0mm, boxsep=1pt, left=2pt, right=2pt, top=1pt, bottom=1pt]
    \begin{verbatim}
Given question & chunk:
1) Summarize chunk relevance.
2) Rate relevance (0-5).

Question: LLM reasoning consistency?
Chunk: [Chunk text...]

Output JSON: { "summary": "...",
"relevance": 0-5 }
    \end{verbatim}
    \end{tcolorbox}
    % Removed vspace

    % --- Section C ---
    \sectiontitlegreen{C) Follow-up Query Prompt (if needed):}
    % Use tcolorbox for light green background and black text
    \begin{tcolorbox}[colback=lightgreenbg, coltext=blacktext, boxrule=0pt, arc=0mm, boxsep=1pt, left=2pt, right=2pt, top=1pt, bottom=1pt]
    \begin{verbatim}
Original Question: LLM reasoning
consistency?
Context Summaries:
[Summary 1 from B]
[Summary 2 from B]
...

Generate specific follow-up query.
Output query text only.
    \end{verbatim}
    \end{tcolorbox}
    % Removed vspace

    % --- Section D ---
    \sectiontitlegreen{D) Final Answer Synthesis Prompt:}
    % Use tcolorbox for light green background and black text
    \begin{tcolorbox}[colback=lightgreenbg, coltext=blacktext, boxrule=0pt, arc=0mm, boxsep=1pt, left=2pt, right=2pt, top=1pt, bottom=1pt]
    \begin{verbatim}
Context:
[Source: paper_1] Summary 1 (R: 5/5)
[Source: search_1] Summary 2 (R: 4/5)
... (final context)

Question: LLM reasoning consistency?

TASK: Answer using ONLY context. Cite
[source_name]. List Sources at end.
    \end{verbatim}
    \end{tcolorbox}
    % Removed vspace

    % --- Section E ---
    \sectiontitlegreen{E) Xplor's Generated Answer:} \\
    Synthesized answer using context from (D) with citations.
    % Use tcolorbox for light green background and black text
    \begin{tcolorbox}[colback=lightgreenbg, coltext=blacktext, boxrule=0pt, arc=0mm, boxsep=1pt, left=2pt, right=2pt, top=1pt, bottom=1pt]
    \begin{verbatim}
LLMs face consistency challenges [paper_1].
Key issue is factual consistency...
Another area is... [search_1].

Sources:
[paper_1]
[search_1]
...
    \end{verbatim}
    \end{tcolorbox}

  \end{minipage}

  \caption{Xplor prompt evolution: (A) Input, (B) Chunk relevance/summary, (C) Optional follow-up query, (D) Final synthesis context, (E) Synthesized answer.}
  \label{fig:xplor_prompt_revised}
\end{figure}
